A Noise is Worth Diffusion Guidance

Diffusion models excel in generating high-quality images. However, current diffusion models struggle to produce reliable images without guidance methods, such as classifier-free guidance (CFG). Are guidance methods truly necessary? Observing that noise obtained via diffusion inversion can reconstruct high-quality images without guidance, we focus on the initial noise of the denoising pipeline. By mapping Gaussian noise to `guidance-free noise', we uncover that small low-magnitude low-frequency components significantly enhance the denoising process, removing the need for guidance and thus improving both inference throughput and memory. Expanding on this, we propose \ours, a novel method that replaces guidance methods with a single refinement of the initial noise. This refined noise enables high-quality image generation without guidance, within the same diffusion pipeline. Our noise-refining model leverages efficient noise-space learning, achieving rapid convergence and strong performance with just 50K text-image pairs. We validate its effectiveness across diverse metrics and analyze how refined noise can eliminate the need for guidance. See our project page: https://cvlab-kaist.github.io/NoiseRefine/.

==> fig/inference/inference.tex <==
% \begin{figure}[!t]
%     \includegraphics[width=\linewidth]{fig/inference/inference.pdf}
%     \caption{
%     \textbf{Inference comparison between \ours and guidance methods.} Thanks to our noise generator, \ours achieves \textbf{\textit{approximately 2x faster}} inference speed compared to guidance methods, while preserving generation quality.
%     }
%     \label{fig:inference}
% \end{figure}

==> fig/noise/noise.tex <==

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.4\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/noise/36.png}
        \caption{Seed 36}
        \label{fig:noise1}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.4\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/noise/96.png}
        \caption{Seed 96}
        \label{fig:noise2}
    \end{subfigure}
    \caption{\textbf{Comparison of generation quality between different noises.} Using the prompt "a photo of a corgi" with the Stable Diffusion v2.1 model, we observe that diffusion models exhibit significant quality variation due to initial noise when no guidance is applied. However, by using the noise generated by our proposed Noise Generator, the model consistently produces high-quality images, even without guidance. This approach demonstrates the capability of our Noise Generator to stabilize output quality, effectively minimizing dependency on guidance for reliable image generation.}
    \label{fig:twofigures}
\end{figure}


% 프롬프트는 'a photo of a corgi'이고, 모델은 Stable Diffusion v2.1이다. Gudiance를 사용하지 않으면, 디퓨전 모델은 initial noise에 따른 퀄리티 편차가 심하다. 우리가 제시하는 Noise Generator의 Noise를 사용하면, Gudiance 없이도 일관되게 좋은 이미지를 생성할 수 있다.

==> fig/noise/teaser.tex <==
  % \begin{figure}[H]
  % \setlength{\linewidth}{\textwidth}    
  % \setlength{\hsize}{\textwidth}
  % \centering
  %   \begin{subfigure}[b]{0.24\linewidth}
  %       \centering
  %       \includegraphics[width=\linewidth]{fig/noise/36.pdf}
  %       \caption{Seed 36}
  %       \label{fig:noise1}
  %   \end{subfigure}
  %   % \hfill
  %   \begin{subfigure}[b]{0.24\linewidth}
  %       \centering
  %       \includegraphics[width=\linewidth]{fig/noise/96.pdf}
  %       \caption{Seed 96}
  %       \label{fig:noise2}
  %   \end{subfigure}
  %   \begin{subfigure}[b]{0.24\linewidth}
  %       \centering
  %       \includegraphics[width=\linewidth]{example-image-a}
  %       \caption{Generated Noise w/ Seed 36}
  %       \label{fig:noise1}
  %   \end{subfigure}
  %   % \hfill
  %   \begin{subfigure}[b]{0.24\linewidth}
  %       \centering
  %       \includegraphics[width=\linewidth]{fig/noise/96_cfg.pdf}
  %       \caption{Generated Noise w/ Seed 96}
  %       \label{fig:noise2}
  %   \end{subfigure}
  %   \caption{\textbf{Comparison of generation quality between different noises.} Using the prompt \textit{``a photo of a corgi''} with the Stable Diffusion~\cite{rombach2022high} v2.1, we observe that diffusion models exhibit significant quality variation due to initial noise when no guidance is applied, as shown in (a) and (b). However, by using the noise generated by our proposed Noise Generator, the model consistently produces high-quality images, even without guidance. This demonstrates the capability of our Noise Generator to stabilize output quality, effectively minimizing dependency on guidance but producing comparable quality.}
  % \end{figure}

% \begin{figure}[H]
%     \setlength{\linewidth}{\textwidth}    
%     \setlength{\hsize}{\textwidth}
%     \begin{minipage}[t]{0.49\linewidth}
%         \includegraphics[width=\linewidth]{example-image-a}
%         \caption{\textbf{Comparison of generation quality between different noises.} Using the prompt \textit{``a photo of a corgi''} with the Stable Diffusion~\cite{rombach2022high} v2.1, we observe that diffusion models exhibit significant quality variation due to initial noise when no guidance is applied, as shown in (a) and (b). However, by using the noise generated by our proposed Noise Generator, the model consistently produces high-quality images, even without guidance. This demonstrates the capability of our Noise Generator to stabilize output quality, effectively minimizing dependency on guidance but producing comparable quality.}
%         \label{fig:images_from_different_noises}
%     \end{minipage} 
% \end{figure}

